Broken Adaptive Ridge in High-Dimensional Vector Autoregressions

We study regularized estimation in high-dimensional vector autoregressions under physical dependence and row-wise approximate sparsity using the Broken Adaptive Ridge (BAR) estimator. BAR is an iteratively reweighted Ridge procedure whose fixed-point first-order conditions imply a coordinatewise thresholding rule that produces exact zeros. We show that the BAR estimation error can be analyzed on the union of the population support above the BAR threshold and the support selected in the sample. The size of this union can be controlled at the rate implied by approximate sparsity, allowing us to establish the required restricted-curvature condition and derive L1, L2, and prediction error rates when the number of regressors grows polynomially with the sample size and may exceed it. Under exact sparsity, the resulting rates recover the familiar rates for sparse high-dimensional estimation. Monte Carlo experiments across a range of high-dimensional VAR designs show that BAR delivers strong estimation and forecasting performance, and retains a high share of relevant coefficients relative to Lasso, adaptive Lasso, and SCAD. An application to U.S. inflation forecasting using FRED-MD shows particularly strong performance at the one-month horizon.

==> Tables/tab_BAR_MD_ebic_CPIAUCSL_lags1_roll0.tex <==
\begin{table}[H]
\centering
\caption{RMSFE and MAFE ratios relative to the AR(1) using an expanding window estimation.}
\label{tab:MD_inflation_lags1_roll0}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccc}
   \toprule
\multirow{2}{*}{period} & \multirow{2}{*}{model} & \multicolumn{2}{c}{h=1} & \multicolumn{2}{c}{h=3} & \multicolumn{2}{c}{h=6} & \multicolumn{2}{c}{h=12} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
{} & {} & RMSFE & MAFE & RMSFE & MAFE & RMSFE & MAFE & RMSFE & MAFE \\ 
 \midrule
\multirow{6}{*}{1990-2019} & BAR & \cellcolor{gray!30}{\underline{\textbf{0.87}}} & \cellcolor{cyan!10}{\underline{\textbf{0.89}}} & \cellcolor{gray!30}{\textbf{0.96}} & \cellcolor{cyan!10}{\textbf{0.95}} & 0.95 & 0.93 & 1.37 & 1.07 \\ 
  {} & aLASSO(ridge) & 0.90 & 0.92 & \textbf{0.96} & \textbf{0.95} & \textbf{0.94} & \textbf{0.92} & \textbf{1.00} & \textbf{1.01} \\ 
  {} & aLASSO(lasso) & 0.91 & 0.93 & \textbf{0.96} & \textbf{0.95} & \textbf{0.94} & \textbf{0.92} & \textbf{1.00} & \textbf{1.01} \\ 
  {} & LASSO & 0.93 & 0.94 & \cellcolor{gray!30}{\textbf{0.96}} & \cellcolor{cyan!10}{\textbf{0.95}} & \cellcolor{gray!30}{\textbf{0.94}} & \cellcolor{cyan!10}{\textbf{0.92}} & \cellcolor{gray!30}{\textbf{1.00}} & \cellcolor{cyan!10}{\textbf{1.01}} \\ 
  {} & SCAD & 0.92 & 0.94 & \cellcolor{gray!30}{\textbf{0.96}} & \cellcolor{cyan!10}{\textbf{0.95}} & \cellcolor{gray!30}{\textbf{0.94}} & \cellcolor{cyan!10}{\textbf{0.92}} & \cellcolor{gray!30}{\textbf{1.00}} & \cellcolor{cyan!10}{\textbf{1.01}} \\ 
   \midrule
\multirow{6}{*}{2020-2021} & BAR & 0.90 & 0.88 & \textbf{1.08} & \textbf{1.06} & \cellcolor{gray!30}{\textbf{0.93}} & \cellcolor{cyan!10}{\textbf{0.91}} & \underline{\textbf{1.01}} & \cellcolor{cyan!10}{\underline{\textbf{1.02}}} \\ 
  {} & aLASSO(ridge) & 0.84 & 0.82 & \textbf{1.08} & \textbf{1.06} & \textbf{0.93} & \textbf{0.91} & 1.03 & 1.03 \\ 
  {} & aLASSO(lasso) & 1.01 & 0.90 & \textbf{1.08} & \textbf{1.06} & \textbf{0.93} & \textbf{0.91} & 1.03 & 1.03 \\ 
  {} & LASSO & \cellcolor{gray!30}{\underline{\textbf{0.76}}} & \cellcolor{cyan!10}{\underline{\textbf{0.73}}} & \textbf{1.08} & \textbf{1.06} & \cellcolor{gray!30}{\textbf{0.93}} & \cellcolor{cyan!10}{\textbf{0.91}} & 1.03 & 1.03 \\ 
  {} & SCAD & 0.82 & 0.83 & \textbf{1.08} & \textbf{1.06} & \cellcolor{gray!30}{\textbf{0.93}} & \cellcolor{cyan!10}{\textbf{0.91}} & 1.03 & 1.03 \\ 
   \midrule
\multirow{6}{*}{2022-2025} & BAR & 0.90 & 0.89 & \cellcolor{gray!30}{\textbf{0.90}} & \cellcolor{cyan!10}{\textbf{0.93}} & \cellcolor{gray!30}{\textbf{1.04}} & \textbf{1.05} & \underline{\textbf{0.93}} & \cellcolor{cyan!10}{\underline{\textbf{0.91}}} \\ 
  {} & aLASSO(ridge) & \underline{\textbf{0.88}} & 0.89 & \textbf{0.90} & \textbf{0.93} & \textbf{1.04} & \textbf{1.05} & 0.95 & 0.97 \\ 
  {} & aLASSO(lasso) & 0.90 & 0.94 & \textbf{0.90} & \textbf{0.93} & \textbf{1.04} & \textbf{1.05} & 0.95 & 0.97 \\ 
  {} & LASSO & 0.93 & 0.95 & \textbf{0.90} & \textbf{0.93} & \cellcolor{gray!30}{\textbf{1.04}} & \textbf{1.05} & \cellcolor{gray!30}{0.95} & 0.97 \\ 
  {} & SCAD & 0.89 & \underline{\textbf{0.88}} & \textbf{0.90} & \textbf{0.93} & \cellcolor{gray!30}{\textbf{1.04}} & \textbf{1.05} & \cellcolor{gray!30}{0.95} & 0.97 \\ 
   \bottomrule
\multicolumn{10}{l}{\begin{minipage}{\dimexpr\columnwidth+13\tabcolsep}
\footnotesize\textit{Notes}: the RMSFE and the MAFE are relative to the AR(1) benchmark. Bold and underlined entries denote the best-performing model(s) for each forecast horizon and period. Grey cells indicate models belonging to the Set of Superior Models (SSM) under the 50\% MCS procedure using the $T_{\text{max}}$ statistic with squared errors, whereas blue cells indicate models included in the SSM when absolute errors are used.
\end{minipage}
}\end{tabular}
} % end resizebox
\end{table}


==> Tables/tab_MC_BAR_ebic_CMP_rho0.5_sparsity_r10_eig_0.75_0.25.tex <==
\begin{table}[H]
\centering
\caption{MC simulations: $r$=10, $\rho$=0.5, EBIC.}
\label{tab:MC_r10_rho0.5}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc}
  \toprule
 & \multicolumn{3}{c}{\multirow{2}{*}{BAR}}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{\multirow{2}{*}{LASSO}}& \multicolumn{3}{c}{\multirow{2}{*}{SCAD}}\\ 
 & \multicolumn{3}{c}{}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Ridge)}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Lasso)}& \multicolumn{3}{c}{}& \multicolumn{3}{c}{}\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 $T$ & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 \\ 
\midrule 
  \addlinespace
$K$ & \multicolumn{15}{c}{\underline{\textit{RMSFE}}}\\ 
 \addlinespace[0.5ex]
 20 & \textbf{0.110} & \textbf{0.107} & \textbf{0.102} & \textbf{0.110} & \textbf{0.107} & \textbf{0.102} & 0.111 & \textbf{0.107} & \textbf{0.102} & 0.112 & 0.109 & 0.103 & 0.111 & \textbf{0.107} & \textbf{0.102} \\ 
   40 & \underline{\textbf{0.111}} & \textbf{0.106} & \textbf{0.102} & 0.113 & \textbf{0.106} & \textbf{0.102} & 0.113 & \textbf{0.106} & \textbf{0.102} & 0.114 & 0.108 & 0.103 & 0.114 & 0.107 & \textbf{0.102} \\ 
   80 & 0.113 & \underline{\textbf{0.106}} & \textbf{0.102} & \underline{\textbf{0.112}} & 0.108 & \textbf{0.102} & 0.114 & 0.107 & \textbf{0.102} & 0.115 & 0.110 & 0.103 & 0.122 & 0.109 & \textbf{0.102} \\ 
  160 & 0.118 & \underline{\textbf{0.106}} & \textbf{0.102} & \underline{\textbf{0.114}} & 0.107 & \textbf{0.102} & 0.115 & 0.107 & \textbf{0.102} & 0.116 & 0.110 & 0.103 & 0.145 & 0.110 & \textbf{0.102} \\ 
  320 & 0.126 & \underline{\textbf{0.107}} & \textbf{0.102} & \underline{\textbf{0.116}} & 0.108 & 0.103 & 0.117 & 0.108 & \textbf{0.102} & 0.117 & 0.111 & 0.104 & 0.146 & 0.111 & 0.103 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{RMSE}}}\\ 
 \addlinespace[0.5ex]
 20 & 1.732 & 1.192 & 0.729 & \underline{\textbf{1.713}} & \underline{\textbf{1.128}} & \underline{\textbf{0.690}} & 1.798 & 1.173 & 0.712 & 1.845 & 1.384 & 0.813 & 1.832 & 1.269 & 0.710 \\ 
   40 & \underline{\textbf{2.610}} & \underline{\textbf{1.711}} & 1.039 & 2.712 & 1.771 & \underline{\textbf{1.000}} & 2.736 & 1.779 & 1.024 & 2.789 & 2.110 & 1.214 & 2.772 & 1.973 & 1.020 \\ 
   80 & 4.094 & \underline{\textbf{2.513}} & 1.486 & \underline{\textbf{3.762}} & 2.941 & \underline{\textbf{1.449}} & 4.042 & 2.713 & 1.464 & 4.109 & 3.193 & 1.797 & 5.561 & 3.051 & 1.476 \\ 
  160 & 6.904 & \underline{\textbf{3.751}} & 2.122 & \underline{\textbf{5.639}} & 3.823 & 2.110 & 5.951 & 4.039 & \underline{\textbf{2.091}} & 6.024 & 4.717 & 2.637 & 11.864 & 4.577 & 2.139 \\ 
  320 & 12.023 & \underline{\textbf{5.864}} & 3.042 & \underline{\textbf{8.398}} & 5.865 & 3.120 & 8.695 & 6.121 & \underline{\textbf{2.981}} & 8.767 & 7.035 & 3.870 & 16.568 & 6.935 & 3.119 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Correct sparsity}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   40 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   80 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{True model included}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   40 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   80 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Share of relevant variables}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.089}} & 0.121 & 0.209 & 0.084 & 0.120 & 0.198 & 0.063 & 0.111 & 0.203 & 0.069 & 0.125 & \underline{\textbf{0.257}} & 0.078 & \underline{\textbf{0.130}} & 0.197 \\ 
   40 & \underline{\textbf{0.083}} & \underline{\textbf{0.114}} & 0.199 & 0.057 & 0.106 & 0.177 & 0.046 & 0.098 & 0.190 & 0.049 & 0.106 & \underline{\textbf{0.229}} & 0.054 & 0.110 & 0.178 \\ 
   80 & \underline{\textbf{0.078}} & \underline{\textbf{0.110}} & 0.191 & 0.055 & 0.089 & 0.159 & 0.036 & 0.087 & 0.179 & 0.037 & 0.091 & \underline{\textbf{0.208}} & 0.057 & 0.094 & 0.163 \\ 
  160 & 0.072 & \underline{\textbf{0.106}} & 0.184 & 0.042 & 0.094 & 0.144 & 0.027 & 0.079 & 0.170 & 0.027 & 0.081 & \underline{\textbf{0.192}} & \underline{\textbf{0.087}} & 0.083 & 0.154 \\ 
  320 & \underline{\textbf{0.063}} & \underline{\textbf{0.101}} & \textbf{0.178} & 0.030 & 0.084 & 0.130 & 0.019 & 0.069 & 0.161 & 0.019 & 0.070 & \textbf{0.178} & 0.062 & 0.072 & 0.147 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Positive Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.012 & 0.008 & \textbf{0.003} & 0.012 & 0.008 & 0.005 & \underline{\textbf{0.005}} & \underline{\textbf{0.005}} & \textbf{0.003} & 0.007 & 0.008 & 0.008 & 0.014 & 0.011 & 0.005 \\ 
   40 & 0.009 & 0.005 & 0.002 & 0.005 & 0.004 & 0.002 & \textbf{0.002} & \underline{\textbf{0.002}} & \textbf{0.001} & \textbf{0.002} & 0.003 & 0.003 & 0.005 & 0.004 & \textbf{0.001} \\ 
   80 & 0.008 & 0.004 & 0.001 & 0.002 & 0.002 & 0.001 & \textbf{0.001} & \textbf{0.001} & 0.001 & \textbf{0.001} & \textbf{0.001} & 0.001 & 0.019 & 0.002 & \underline{\textbf{0.000}} \\ 
  160 & 0.008 & 0.003 & 0.001 & 0.001 & 0.001 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & 0.048 & 0.001 & \textbf{0.000} \\ 
  320 & 0.008 & 0.002 & 0.001 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & 0.029 & \textbf{0.000} & \textbf{0.000} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Negative Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.911}} & 0.879 & 0.791 & 0.916 & 0.880 & 0.802 & 0.937 & 0.889 & 0.797 & 0.931 & 0.875 & \underline{\textbf{0.743}} & 0.922 & \underline{\textbf{0.870}} & 0.803 \\ 
   40 & \underline{\textbf{0.917}} & \underline{\textbf{0.886}} & 0.801 & 0.943 & 0.894 & 0.823 & 0.954 & 0.902 & 0.810 & 0.951 & 0.894 & \underline{\textbf{0.771}} & 0.946 & 0.890 & 0.822 \\ 
   80 & \underline{\textbf{0.922}} & \underline{\textbf{0.890}} & 0.809 & 0.945 & 0.911 & 0.841 & 0.964 & 0.913 & 0.821 & 0.963 & 0.909 & \underline{\textbf{0.792}} & 0.943 & 0.906 & 0.837 \\ 
  160 & 0.928 & \underline{\textbf{0.894}} & 0.816 & 0.958 & 0.906 & 0.856 & 0.973 & 0.921 & 0.830 & 0.973 & 0.919 & \underline{\textbf{0.808}} & \underline{\textbf{0.913}} & 0.917 & 0.846 \\ 
  320 & \underline{\textbf{0.937}} & \underline{\textbf{0.899}} & \textbf{0.822} & 0.970 & 0.916 & 0.870 & 0.981 & 0.931 & 0.839 & 0.981 & 0.930 & \textbf{0.822} & 0.938 & 0.928 & 0.853 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Number of variables}}}\\ 
 \addlinespace[0.5ex]
 20 & 1.009 & 1.286 & 2.118 & 0.966 & 1.279 & 2.029 & 0.676 & 1.157 & 2.061 & 0.758 & 1.329 & 2.651 & 0.920 & 1.408 & 2.024 \\ 
   40 & 1.110 & 1.290 & 2.050 & 0.734 & 1.181 & 1.835 & 0.518 & 1.042 & 1.937 & 0.558 & 1.140 & 2.376 & 0.678 & 1.228 & 1.814 \\ 
   80 & 1.345 & 1.349 & 1.997 & 0.702 & 1.054 & 1.649 & 0.400 & 0.932 & 1.829 & 0.418 & 0.985 & 2.155 & 1.895 & 1.067 & 1.665 \\ 
  160 & 1.941 & 1.455 & 1.961 & 0.563 & 1.060 & 1.490 & 0.299 & 0.843 & 1.742 & 0.307 & 0.872 & 1.987 & 8.140 & 0.940 & 1.571 \\ 
  320 & 3.049 & 1.675 & 1.938 & 0.415 & 0.964 & 1.350 & 0.211 & 0.739 & 1.651 & 0.215 & 0.755 & 1.837 & 9.518 & 0.840 & 1.496 \\ 
   \bottomrule
\end{tabular}
} % end resizebox
\end{table}


==> Tables/tab_MC_BAR_ebic_CMP_rho0.5_sparsity_r1_eig_0.75_0.25.tex <==
\begin{table}[H]
\centering
\caption{MC simulations: $r$=1, $\rho$=0.5, EBIC.}
\label{tab:MC_r1_rho0.5}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc}
  \toprule
 & \multicolumn{3}{c}{\multirow{2}{*}{BAR}}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{\multirow{2}{*}{LASSO}}& \multicolumn{3}{c}{\multirow{2}{*}{SCAD}}\\ 
 & \multicolumn{3}{c}{}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Ridge)}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Lasso)}& \multicolumn{3}{c}{}& \multicolumn{3}{c}{}\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 $T$ & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 \\ 
\midrule 
  \addlinespace
$K$ & \multicolumn{15}{c}{\underline{\textit{RMSFE}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.109}} & 0.105 & \textbf{0.101} & 0.111 & 0.105 & \textbf{0.101} & 0.110 & \underline{\textbf{0.104}} & \textbf{0.101} & 0.111 & 0.107 & \textbf{0.101} & 0.110 & 0.106 & \textbf{0.101} \\ 
   40 & \underline{\textbf{0.112}} & \textbf{0.104} & \textbf{0.100} & 0.115 & 0.107 & 0.101 & 0.113 & \textbf{0.104} & \textbf{0.100} & 0.113 & 0.107 & 0.101 & 0.113 & 0.106 & \textbf{0.100} \\ 
   80 & 0.115 & \underline{\textbf{0.104}} & \textbf{0.100} & \underline{\textbf{0.113}} & 0.112 & 0.101 & 0.114 & 0.106 & \textbf{0.100} & 0.114 & 0.108 & 0.101 & 0.120 & 0.107 & \textbf{0.100} \\ 
  160 & 0.121 & \underline{\textbf{0.105}} & \textbf{0.100} & \textbf{0.114} & 0.107 & 0.101 & 0.115 & 0.106 & \textbf{0.100} & \textbf{0.114} & 0.109 & 0.101 & 0.141 & 0.109 & \textbf{0.100} \\ 
  320 & 0.128 & \textbf{0.108} & \textbf{0.100} & \textbf{0.116} & 0.109 & 0.102 & \textbf{0.116} & \textbf{0.108} & \textbf{0.100} & \textbf{0.116} & 0.110 & 0.101 & 0.143 & 0.110 & \textbf{0.100} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{RMSE}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{1.852}} & 1.057 & 0.220 & 1.966 & 1.107 & 0.228 & 1.856 & \underline{\textbf{0.946}} & 0.210 & 1.876 & 1.262 & 0.481 & 1.915 & 1.104 & \underline{\textbf{0.182}} \\ 
   40 & 2.982 & \underline{\textbf{1.561}} & 0.330 & 3.086 & 2.118 & 0.345 & \underline{\textbf{2.831}} & 1.566 & 0.309 & 2.836 & 2.001 & 0.750 & 2.911 & 1.843 & \underline{\textbf{0.263}} \\ 
   80 & 5.153 & \underline{\textbf{2.395}} & 0.497 & \underline{\textbf{4.137}} & 3.887 & 0.559 & 4.197 & 2.539 & 0.458 & 4.172 & 3.109 & 1.157 & 5.878 & 2.969 & \underline{\textbf{0.396}} \\ 
  160 & 9.135 & 3.981 & 0.743 & 6.207 & 4.173 & 1.018 & 6.140 & \underline{\textbf{3.960}} & 0.670 & \underline{\textbf{6.085}} & 4.702 & 1.761 & 13.293 & 4.593 & \underline{\textbf{0.604}} \\ 
  320 & 15.026 & 7.467 & 1.133 & 9.056 & 6.995 & 2.818 & 8.860 & \underline{\textbf{6.234}} & 0.971 & \underline{\textbf{8.766}} & 7.126 & 2.663 & 19.094 & 7.099 & \underline{\textbf{0.965}} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Correct sparsity}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & \underline{\textbf{0.010}} & 0.452 & 0.000 & 0.000 & 0.599 & 0.000 & 0.008 & 0.512 & 0.000 & 0.000 & 0.038 & 0.000 & 0.000 & \underline{\textbf{0.840}} \\ 
   40 & 0.000 & 0.000 & 0.123 & 0.000 & 0.000 & 0.347 & 0.000 & 0.000 & 0.193 & 0.000 & 0.000 & 0.009 & 0.000 & 0.000 & \underline{\textbf{0.702}} \\ 
   80 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.086 & 0.000 & 0.000 & 0.020 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \underline{\textbf{0.464}} \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \underline{\textbf{0.128}} \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \underline{\textbf{0.003}} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{True model included}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.100 & 0.995 & 0.000 & 0.091 & \textbf{1.000} & 0.000 & 0.098 & \textbf{1.000} & 0.000 & 0.102 & \textbf{1.000} & 0.000 & \underline{\textbf{0.107}} & \textbf{1.000} \\ 
   40 & 0.000 & \underline{\textbf{0.008}} & 0.986 & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} \\ 
   80 & 0.000 & 0.000 & 0.966 & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} \\ 
  160 & 0.000 & 0.000 & 0.942 & 0.000 & 0.000 & 0.998 & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} \\ 
  320 & 0.000 & 0.000 & 0.902 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Share of relevant variables}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.531}} & 0.850 & \textbf{1.000} & 0.401 & \underline{\textbf{0.893}} & \textbf{1.000} & 0.410 & 0.884 & \textbf{1.000} & 0.418 & 0.886 & \textbf{1.000} & 0.435 & 0.891 & \textbf{1.000} \\ 
   40 & \underline{\textbf{0.478}} & \underline{\textbf{0.853}} & \textbf{1.000} & 0.173 & 0.708 & \textbf{1.000} & 0.283 & 0.816 & \textbf{1.000} & 0.287 & 0.819 & \textbf{1.000} & 0.298 & 0.826 & \textbf{1.000} \\ 
   80 & \underline{\textbf{0.375}} & \underline{\textbf{0.845}} & \textbf{1.000} & 0.274 & 0.356 & \textbf{1.000} & 0.194 & 0.734 & \textbf{1.000} & 0.197 & 0.735 & \textbf{1.000} & 0.213 & 0.743 & \textbf{1.000} \\ 
  160 & \underline{\textbf{0.223}} & \underline{\textbf{0.813}} & \textbf{1.000} & 0.138 & 0.736 & \textbf{1.000} & 0.116 & 0.657 & \textbf{1.000} & 0.117 & 0.658 & \textbf{1.000} & 0.165 & 0.664 & \textbf{1.000} \\ 
  320 & 0.089 & \underline{\textbf{0.721}} & \textbf{1.000} & 0.046 & 0.545 & 0.981 & 0.065 & 0.556 & \textbf{1.000} & 0.065 & 0.557 & \textbf{1.000} & \underline{\textbf{0.105}} & 0.564 & \textbf{1.000} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Positive Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.018 & 0.008 & 0.002 & 0.022 & 0.016 & 0.002 & \underline{\textbf{0.008}} & \underline{\textbf{0.007}} & 0.002 & 0.011 & 0.015 & 0.009 & 0.020 & 0.018 & \underline{\textbf{0.001}} \\ 
   40 & 0.015 & 0.006 & 0.002 & 0.009 & 0.011 & 0.001 & \underline{\textbf{0.003}} & \underline{\textbf{0.003}} & 0.001 & 0.004 & 0.006 & 0.004 & 0.008 & 0.008 & \underline{\textbf{0.000}} \\ 
   80 & 0.015 & 0.004 & 0.001 & 0.004 & 0.005 & \textbf{0.000} & \textbf{0.001} & \textbf{0.002} & 0.001 & \textbf{0.001} & \textbf{0.002} & 0.002 & 0.020 & 0.003 & \textbf{0.000} \\ 
  160 & 0.014 & 0.004 & 0.001 & 0.002 & 0.002 & \textbf{0.000} & \textbf{0.000} & \textbf{0.001} & \textbf{0.000} & \textbf{0.000} & \textbf{0.001} & 0.001 & 0.052 & \textbf{0.001} & \textbf{0.000} \\ 
  320 & 0.011 & 0.004 & \textbf{0.000} & 0.001 & 0.001 & 0.001 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & 0.033 & 0.001 & \textbf{0.000} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Negative Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.469}} & 0.150 & 0.000 & 0.599 & \underline{\textbf{0.107}} & 0.000 & 0.590 & 0.116 & 0.000 & 0.582 & 0.114 & 0.000 & 0.565 & 0.109 & 0.000 \\ 
   40 & \underline{\textbf{0.522}} & \underline{\textbf{0.147}} & 0.000 & 0.827 & 0.292 & 0.000 & 0.717 & 0.184 & 0.000 & 0.713 & 0.181 & 0.000 & 0.702 & 0.174 & 0.000 \\ 
   80 & \underline{\textbf{0.625}} & \underline{\textbf{0.155}} & 0.000 & 0.726 & 0.644 & 0.000 & 0.806 & 0.266 & 0.000 & 0.803 & 0.265 & 0.000 & 0.787 & 0.257 & 0.000 \\ 
  160 & \underline{\textbf{0.777}} & \underline{\textbf{0.187}} & 0.000 & 0.862 & 0.264 & 0.000 & 0.884 & 0.343 & 0.000 & 0.883 & 0.342 & 0.000 & 0.835 & 0.336 & 0.000 \\ 
  320 & 0.911 & \underline{\textbf{0.279}} & \textbf{0.000} & 0.954 & 0.455 & 0.019 & 0.935 & 0.444 & \textbf{0.000} & 0.935 & 0.443 & \textbf{0.000} & \underline{\textbf{0.895}} & 0.436 & \textbf{0.000} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Number of variables}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.868 & 0.995 & 1.045 & 0.827 & 1.189 & 1.029 & 0.556 & 1.018 & 1.036 & 0.632 & 1.165 & 1.169 & 0.808 & 1.224 & 1.010 \\ 
   40 & 1.074 & 1.071 & 1.060 & 0.527 & 1.124 & 1.030 & 0.391 & 0.952 & 1.046 & 0.428 & 1.048 & 1.141 & 0.601 & 1.142 & 1.010 \\ 
   80 & 1.542 & 1.178 & 1.077 & 0.588 & 0.737 & 1.034 & 0.280 & 0.856 & 1.053 & 0.297 & 0.910 & 1.119 & 1.772 & 1.001 & 1.011 \\ 
  160 & 2.503 & 1.396 & 1.102 & 0.406 & 1.027 & 1.055 & 0.173 & 0.763 & 1.059 & 0.180 & 0.792 & 1.100 & 8.361 & 0.856 & 1.013 \\ 
  320 & 3.545 & 1.983 & 1.138 & 0.256 & 0.838 & 1.303 & 0.103 & 0.639 & 1.062 & 0.106 & 0.654 & 1.087 & 10.633 & 0.743 & 1.017 \\ 
   \bottomrule
\end{tabular}
} % end resizebox
\end{table}


==> Tables/tab_MC_BAR_ebic_CMP_rho0.5_sparsity_r2_eig_0.75_0.25.tex <==
\begin{table}[H]
\centering
\caption{MC simulations: $r$=2, $\rho$=0.5, EBIC.}
\label{tab:MC_r2_rho0.5}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc}
  \toprule
 & \multicolumn{3}{c}{\multirow{2}{*}{BAR}}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{\multirow{2}{*}{LASSO}}& \multicolumn{3}{c}{\multirow{2}{*}{SCAD}}\\ 
 & \multicolumn{3}{c}{}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Ridge)}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Lasso)}& \multicolumn{3}{c}{}& \multicolumn{3}{c}{}\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 $T$ & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 \\ 
\midrule 
  \addlinespace
$K$ & \multicolumn{15}{c}{\underline{\textit{RMSFE}}}\\ 
 \addlinespace[0.5ex]
 20 & \textbf{0.112} & \textbf{0.107} & \textbf{0.101} & \textbf{0.112} & \textbf{0.107} & \textbf{0.101} & 0.114 & 0.108 & \textbf{0.101} & 0.114 & 0.109 & 0.102 & 0.114 & 0.108 & \textbf{0.101} \\ 
   40 & \underline{\textbf{0.113}} & \underline{\textbf{0.106}} & \textbf{0.101} & 0.114 & 0.107 & \textbf{0.101} & 0.115 & 0.108 & \textbf{0.101} & 0.115 & 0.110 & 0.102 & 0.115 & 0.109 & \textbf{0.101} \\ 
   80 & 0.115 & \underline{\textbf{0.107}} & \textbf{0.101} & \underline{\textbf{0.114}} & 0.110 & \textbf{0.101} & 0.115 & 0.109 & \textbf{0.101} & 0.115 & 0.111 & 0.103 & 0.125 & 0.111 & \textbf{0.101} \\ 
  160 & 0.120 & \underline{\textbf{0.108}} & \underline{\textbf{0.100}} & \underline{\textbf{0.115}} & 0.109 & 0.102 & 0.116 & 0.110 & 0.101 & 0.116 & 0.112 & 0.103 & 0.149 & 0.112 & 0.101 \\ 
  320 & 0.128 & \underline{\textbf{0.109}} & \underline{\textbf{0.100}} & \underline{\textbf{0.116}} & 0.110 & 0.103 & 0.117 & 0.111 & 0.101 & 0.117 & 0.113 & 0.103 & 0.149 & 0.113 & 0.101 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{RMSE}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{1.980}} & \underline{\textbf{1.315}} & \underline{\textbf{0.291}} & 2.018 & 1.375 & 0.373 & 2.119 & 1.435 & 0.319 & 2.157 & 1.672 & 0.691 & 2.134 & 1.539 & 0.399 \\ 
   40 & \underline{\textbf{3.016}} & \underline{\textbf{1.946}} & \underline{\textbf{0.429}} & 3.119 & 2.229 & 0.601 & 3.172 & 2.251 & 0.493 & 3.211 & 2.589 & 1.116 & 3.199 & 2.460 & 0.659 \\ 
   80 & 4.764 & \underline{\textbf{2.936}} & \underline{\textbf{0.646}} & \underline{\textbf{4.429}} & 3.675 & 1.030 & 4.647 & 3.487 & 0.804 & 4.685 & 3.932 & 1.775 & 6.271 & 3.824 & 1.084 \\ 
  160 & 7.894 & \underline{\textbf{4.521}} & \underline{\textbf{0.966}} & \underline{\textbf{6.533}} & 4.994 & 1.968 & 6.760 & 5.240 & 1.292 & 6.786 & 5.812 & 2.763 & 13.031 & 5.728 & 1.742 \\ 
  320 & 13.313 & \underline{\textbf{7.195}} & \underline{\textbf{1.465}} & \underline{\textbf{9.527}} & 7.569 & 4.069 & 9.736 & 7.904 & 2.098 & 9.749 & 8.595 & 4.243 & 17.969 & 8.572 & 2.774 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Correct sparsity}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & \underline{\textbf{0.423}} & 0.000 & 0.000 & 0.208 & 0.000 & 0.000 & 0.225 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.077 \\ 
   40 & 0.000 & 0.000 & \underline{\textbf{0.088}} & 0.000 & 0.000 & 0.021 & 0.000 & 0.000 & 0.023 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 \\ 
   80 & 0.000 & 0.000 & \underline{\textbf{0.001}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{True model included}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & \underline{\textbf{0.955}} & 0.000 & 0.000 & 0.893 & 0.000 & 0.000 & 0.788 & 0.000 & 0.000 & 0.792 & 0.000 & 0.000 & 0.817 \\ 
   40 & 0.000 & 0.000 & \underline{\textbf{0.904}} & 0.000 & 0.000 & 0.618 & 0.000 & 0.000 & 0.385 & 0.000 & 0.000 & 0.385 & 0.000 & 0.000 & 0.543 \\ 
   80 & 0.000 & 0.000 & \underline{\textbf{0.705}} & 0.000 & 0.000 & 0.059 & 0.000 & 0.000 & 0.020 & 0.000 & 0.000 & 0.020 & 0.000 & 0.000 & 0.134 \\ 
  160 & 0.000 & 0.000 & \underline{\textbf{0.401}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 \\ 
  320 & 0.000 & 0.000 & \underline{\textbf{0.070}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Share of relevant variables}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.366}} & \underline{\textbf{0.640}} & \underline{\textbf{0.999}} & 0.306 & 0.605 & 0.997 & 0.231 & 0.541 & 0.994 & 0.234 & 0.544 & 0.994 & 0.263 & 0.587 & 0.995 \\ 
   40 & \underline{\textbf{0.339}} & \underline{\textbf{0.617}} & \underline{\textbf{0.999}} & 0.194 & 0.503 & 0.994 & 0.157 & 0.454 & 0.988 & 0.158 & 0.455 & 0.988 & 0.174 & 0.489 & 0.992 \\ 
   80 & \underline{\textbf{0.299}} & \underline{\textbf{0.587}} & \underline{\textbf{0.998}} & 0.188 & 0.377 & 0.981 & 0.110 & 0.375 & 0.974 & 0.110 & 0.376 & 0.974 & 0.144 & 0.397 & 0.987 \\ 
  160 & \underline{\textbf{0.260}} & \underline{\textbf{0.555}} & \underline{\textbf{0.997}} & 0.131 & 0.409 & 0.928 & 0.071 & 0.318 & 0.958 & 0.071 & 0.318 & 0.958 & 0.190 & 0.330 & 0.980 \\ 
  320 & \underline{\textbf{0.214}} & \underline{\textbf{0.520}} & \underline{\textbf{0.996}} & 0.086 & 0.350 & 0.730 & 0.045 & 0.258 & 0.934 & 0.045 & 0.258 & 0.934 & 0.149 & 0.266 & 0.970 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Positive Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.015 & 0.010 & \underline{\textbf{0.002}} & 0.013 & 0.011 & 0.004 & \underline{\textbf{0.005}} & \underline{\textbf{0.007}} & 0.004 & 0.007 & 0.013 & 0.020 & 0.013 & 0.017 & 0.007 \\ 
   40 & 0.012 & 0.007 & \textbf{0.002} & 0.005 & 0.006 & 0.003 & \textbf{0.002} & \underline{\textbf{0.003}} & \textbf{0.002} & \textbf{0.002} & 0.004 & 0.009 & 0.004 & 0.007 & 0.004 \\ 
   80 & 0.010 & 0.005 & \textbf{0.001} & 0.002 & 0.003 & 0.002 & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & 0.004 & 0.022 & 0.002 & 0.002 \\ 
  160 & 0.010 & 0.004 & \textbf{0.001} & 0.001 & 0.001 & \textbf{0.001} & \textbf{0.000} & \textbf{0.000} & \textbf{0.001} & \textbf{0.000} & \textbf{0.000} & 0.002 & 0.056 & 0.001 & \textbf{0.001} \\ 
  320 & 0.009 & 0.003 & \textbf{0.000} & \textbf{0.000} & 0.001 & 0.001 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & 0.001 & 0.032 & \textbf{0.000} & 0.001 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Negative Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.634}} & \underline{\textbf{0.360}} & \underline{\textbf{0.001}} & 0.694 & 0.395 & 0.003 & 0.769 & 0.459 & 0.006 & 0.766 & 0.456 & 0.006 & 0.737 & 0.413 & 0.005 \\ 
   40 & \underline{\textbf{0.661}} & \underline{\textbf{0.383}} & \underline{\textbf{0.001}} & 0.806 & 0.497 & 0.006 & 0.843 & 0.546 & 0.012 & 0.842 & 0.545 & 0.012 & 0.826 & 0.511 & 0.008 \\ 
   80 & \underline{\textbf{0.701}} & \underline{\textbf{0.413}} & \underline{\textbf{0.002}} & 0.812 & 0.623 & 0.019 & 0.890 & 0.625 & 0.026 & 0.890 & 0.624 & 0.026 & 0.856 & 0.603 & 0.013 \\ 
  160 & \underline{\textbf{0.740}} & \underline{\textbf{0.445}} & \underline{\textbf{0.003}} & 0.869 & 0.591 & 0.072 & 0.929 & 0.682 & 0.042 & 0.929 & 0.682 & 0.042 & 0.810 & 0.670 & 0.020 \\ 
  320 & \underline{\textbf{0.786}} & \underline{\textbf{0.480}} & \underline{\textbf{0.004}} & 0.914 & 0.650 & 0.270 & 0.955 & 0.742 & 0.066 & 0.955 & 0.742 & 0.066 & 0.851 & 0.734 & 0.030 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Number of variables}}}\\ 
 \addlinespace[0.5ex]
 20 & 1.006 & 1.456 & 2.043 & 0.851 & 1.415 & 2.072 & 0.559 & 1.213 & 2.054 & 0.600 & 1.316 & 2.352 & 0.760 & 1.487 & 2.118 \\ 
   40 & 1.137 & 1.490 & 2.061 & 0.585 & 1.228 & 2.084 & 0.379 & 1.019 & 2.059 & 0.396 & 1.070 & 2.310 & 0.510 & 1.228 & 2.126 \\ 
   80 & 1.384 & 1.546 & 2.082 & 0.553 & 0.959 & 2.091 & 0.264 & 0.838 & 2.049 & 0.270 & 0.862 & 2.248 & 2.013 & 0.969 & 2.123 \\ 
  160 & 2.035 & 1.677 & 2.107 & 0.404 & 1.002 & 2.047 & 0.171 & 0.704 & 2.031 & 0.174 & 0.715 & 2.179 & 9.266 & 0.780 & 2.113 \\ 
  320 & 3.167 & 1.972 & 2.143 & 0.280 & 0.859 & 1.670 & 0.107 & 0.566 & 1.991 & 0.108 & 0.571 & 2.102 & 10.541 & 0.658 & 2.101 \\ 
   \bottomrule
\end{tabular}
} % end resizebox
\end{table}


==> Tables/tab_MC_BAR_ebic_CMP_rho0.5_sparsity_r5_eig_0.75_0.25.tex <==
\begin{table}[H]
\centering
\caption{MC simulations: $r$=5, $\rho$=0.5, EBIC.}
\label{tab:MC_r5_rho0.5}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc}
  \toprule
 & \multicolumn{3}{c}{\multirow{2}{*}{BAR}}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{\multirow{2}{*}{LASSO}}& \multicolumn{3}{c}{\multirow{2}{*}{SCAD}}\\ 
 & \multicolumn{3}{c}{}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Ridge)}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Lasso)}& \multicolumn{3}{c}{}& \multicolumn{3}{c}{}\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 $T$ & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 \\ 
\midrule 
  \addlinespace
$K$ & \multicolumn{15}{c}{\underline{\textit{RMSFE}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.113}} & \underline{\textbf{0.109}} & \underline{\textbf{0.101}} & 0.114 & 0.110 & 0.102 & 0.115 & 0.112 & 0.102 & 0.115 & 0.113 & 0.102 & 0.114 & 0.111 & 0.102 \\ 
   40 & \textbf{0.116} & \underline{\textbf{0.108}} & \textbf{0.101} & \textbf{0.116} & 0.110 & 0.102 & 0.117 & 0.112 & \textbf{0.101} & \textbf{0.116} & 0.113 & 0.103 & \textbf{0.116} & 0.112 & 0.102 \\ 
   80 & 0.118 & \underline{\textbf{0.109}} & \underline{\textbf{0.101}} & \underline{\textbf{0.115}} & 0.113 & 0.102 & 0.116 & 0.114 & 0.102 & 0.116 & 0.114 & 0.104 & 0.129 & 0.113 & 0.102 \\ 
  160 & 0.123 & \underline{\textbf{0.110}} & \underline{\textbf{0.101}} & \textbf{0.116} & 0.113 & 0.102 & \textbf{0.116} & 0.114 & 0.102 & \textbf{0.116} & 0.115 & 0.104 & 0.154 & 0.114 & 0.102 \\ 
  320 & 0.131 & \underline{\textbf{0.112}} & \underline{\textbf{0.101}} & \textbf{0.117} & 0.114 & 0.103 & \textbf{0.117} & 0.115 & 0.102 & \textbf{0.117} & 0.115 & 0.104 & 0.152 & 0.115 & 0.103 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{RMSE}}}\\ 
 \addlinespace[0.5ex]
 20 & 2.209 & \underline{\textbf{1.642}} & \underline{\textbf{0.613}} & \underline{\textbf{2.173}} & 1.679 & 0.630 & 2.296 & 1.935 & 0.629 & 2.256 & 1.975 & 0.865 & 2.256 & 1.882 & 0.682 \\ 
   40 & 3.315 & \underline{\textbf{2.440}} & \underline{\textbf{0.887}} & \underline{\textbf{3.223}} & 2.643 & 0.957 & 3.311 & 2.934 & 0.955 & 3.262 & 2.982 & 1.403 & 3.272 & 2.905 & 1.055 \\ 
   80 & 5.153 & \underline{\textbf{3.657}} & \underline{\textbf{1.295}} & \underline{\textbf{4.628}} & 4.165 & 1.477 & 4.729 & 4.334 & 1.457 & 4.670 & 4.387 & 2.210 & 6.869 & 4.334 & 1.642 \\ 
  160 & 8.416 & \underline{\textbf{5.560}} & \underline{\textbf{1.892}} & \underline{\textbf{6.648}} & 5.979 & 2.336 & 6.722 & 6.288 & 2.225 & 6.653 & 6.342 & 3.410 & 13.866 & 6.313 & 2.574 \\ 
  320 & 14.003 & \underline{\textbf{8.658}} & \underline{\textbf{2.771}} & 9.483 & 8.788 & 3.963 & 9.524 & 9.080 & 3.397 & \underline{\textbf{9.448}} & 9.132 & 5.198 & 18.678 & 9.232 & 4.046 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Correct sparsity}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   40 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   80 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{True model included}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   40 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   80 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Share of relevant variables}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.151}} & \underline{\textbf{0.295}} & 0.572 & 0.109 & 0.278 & 0.596 & 0.057 & 0.183 & 0.590 & 0.060 & 0.199 & \underline{\textbf{0.677}} & 0.083 & 0.236 & 0.615 \\ 
   40 & \underline{\textbf{0.133}} & \underline{\textbf{0.274}} & 0.562 & 0.056 & 0.204 & 0.575 & 0.032 & 0.124 & 0.572 & 0.033 & 0.131 & \underline{\textbf{0.643}} & 0.043 & 0.154 & 0.600 \\ 
   80 & \underline{\textbf{0.112}} & \underline{\textbf{0.253}} & 0.552 & 0.042 & 0.121 & 0.552 & 0.019 & 0.085 & 0.553 & 0.019 & 0.089 & \underline{\textbf{0.610}} & 0.061 & 0.099 & 0.585 \\ 
  160 & 0.092 & \underline{\textbf{0.229}} & 0.543 & 0.023 & 0.114 & 0.527 & 0.010 & 0.062 & 0.533 & 0.010 & 0.063 & \underline{\textbf{0.579}} & \underline{\textbf{0.112}} & 0.068 & 0.571 \\ 
  320 & \underline{\textbf{0.072}} & \underline{\textbf{0.205}} & 0.533 & 0.012 & 0.077 & 0.488 & 0.005 & 0.042 & 0.512 & 0.005 & 0.043 & 0.549 & 0.071 & 0.046 & \underline{\textbf{0.553}} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Positive Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.015 & 0.009 & \underline{\textbf{0.003}} & 0.011 & 0.012 & 0.007 & \underline{\textbf{0.003}} & \underline{\textbf{0.005}} & 0.005 & 0.004 & 0.010 & 0.031 & 0.010 & 0.018 & 0.014 \\ 
   40 & 0.011 & 0.007 & \underline{\textbf{0.002}} & 0.004 & 0.005 & 0.004 & \textbf{0.001} & \textbf{0.002} & 0.003 & \textbf{0.001} & \textbf{0.002} & 0.012 & 0.003 & 0.006 & 0.007 \\ 
   80 & 0.010 & 0.005 & \textbf{0.001} & 0.002 & 0.002 & 0.002 & \textbf{0.000} & \textbf{0.001} & \textbf{0.001} & \textbf{0.000} & \textbf{0.001} & 0.005 & 0.032 & 0.002 & 0.004 \\ 
  160 & 0.010 & 0.004 & \textbf{0.001} & 0.001 & 0.001 & \textbf{0.001} & \textbf{0.000} & \textbf{0.000} & \textbf{0.001} & \textbf{0.000} & \textbf{0.000} & 0.002 & 0.067 & \textbf{0.000} & 0.002 \\ 
  320 & 0.009 & 0.003 & 0.001 & \textbf{0.000} & \textbf{0.000} & 0.001 & \textbf{0.000} & \textbf{0.000} & \underline{\textbf{0.000}} & \textbf{0.000} & \textbf{0.000} & 0.001 & 0.036 & 0.001 & 0.001 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Negative Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.849}} & \underline{\textbf{0.705}} & 0.428 & 0.891 & 0.722 & 0.404 & 0.943 & 0.817 & 0.410 & 0.940 & 0.801 & \underline{\textbf{0.323}} & 0.917 & 0.764 & 0.385 \\ 
   40 & \underline{\textbf{0.867}} & \underline{\textbf{0.726}} & 0.438 & 0.944 & 0.796 & 0.425 & 0.968 & 0.876 & 0.428 & 0.967 & 0.869 & \underline{\textbf{0.357}} & 0.957 & 0.846 & 0.400 \\ 
   80 & \underline{\textbf{0.888}} & \underline{\textbf{0.747}} & 0.448 & 0.958 & 0.879 & 0.448 & 0.981 & 0.915 & 0.447 & 0.981 & 0.911 & \underline{\textbf{0.390}} & 0.939 & 0.901 & 0.415 \\ 
  160 & 0.908 & \underline{\textbf{0.771}} & 0.457 & 0.977 & 0.886 & 0.473 & 0.990 & 0.938 & 0.467 & 0.990 & 0.937 & \underline{\textbf{0.421}} & \underline{\textbf{0.888}} & 0.932 & 0.429 \\ 
  320 & \underline{\textbf{0.928}} & \underline{\textbf{0.795}} & 0.467 & 0.988 & 0.923 & 0.512 & 0.995 & 0.958 & 0.488 & 0.995 & 0.957 & 0.451 & 0.929 & 0.954 & \underline{\textbf{0.447}} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Number of variables}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.975 & 1.615 & 2.911 & 0.707 & 1.574 & 3.087 & 0.330 & 0.988 & 3.025 & 0.364 & 1.138 & 3.843 & 0.569 & 1.444 & 3.281 \\ 
   40 & 1.060 & 1.600 & 2.881 & 0.415 & 1.211 & 3.003 & 0.193 & 0.675 & 2.952 & 0.205 & 0.744 & 3.648 & 0.321 & 0.966 & 3.249 \\ 
   80 & 1.303 & 1.628 & 2.861 & 0.338 & 0.761 & 2.914 & 0.119 & 0.465 & 2.879 & 0.124 & 0.496 & 3.444 & 2.688 & 0.613 & 3.224 \\ 
  160 & 1.980 & 1.712 & 2.846 & 0.221 & 0.703 & 2.821 & 0.069 & 0.335 & 2.788 & 0.071 & 0.350 & 3.242 & 10.889 & 0.403 & 3.204 \\ 
  320 & 3.186 & 1.992 & 2.845 & 0.144 & 0.492 & 2.700 & 0.040 & 0.230 & 2.688 & 0.041 & 0.236 & 3.041 & 11.543 & 0.409 & 3.159 \\ 
   \bottomrule
\end{tabular}
} % end resizebox
\end{table}


==> Tables/tab_MC_BAR_ebic_CMP_rho0_sparsity_r10_eig_0.75_0.25.tex <==
\begin{table}[H]
\centering
\caption{MC simulations: $r$=10, $\rho$=0, EBIC.}
\label{tab:MC_r10_rho0}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc}
  \toprule
 & \multicolumn{3}{c}{\multirow{2}{*}{BAR}}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{\multirow{2}{*}{LASSO}}& \multicolumn{3}{c}{\multirow{2}{*}{SCAD}}\\ 
 & \multicolumn{3}{c}{}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Ridge)}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Lasso)}& \multicolumn{3}{c}{}& \multicolumn{3}{c}{}\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 $T$ & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 \\ 
\midrule 
  \addlinespace
$K$ & \multicolumn{15}{c}{\underline{\textit{RMSFE}}}\\ 
 \addlinespace[0.5ex]
 20 & \textbf{0.109} & \textbf{0.105} & \textbf{0.101} & \textbf{0.109} & \textbf{0.105} & \textbf{0.101} & 0.110 & \textbf{0.105} & \textbf{0.101} & 0.112 & 0.107 & 0.102 & 0.111 & 0.106 & \textbf{0.101} \\ 
   40 & \underline{\textbf{0.110}} & \textbf{0.104} & \textbf{0.102} & 0.113 & 0.105 & \textbf{0.102} & 0.113 & \textbf{0.104} & \textbf{0.102} & 0.114 & 0.107 & 0.103 & 0.114 & 0.106 & \textbf{0.102} \\ 
   80 & \textbf{0.112} & \textbf{0.105} & \textbf{0.102} & \textbf{0.112} & 0.107 & \textbf{0.102} & 0.114 & \textbf{0.105} & \textbf{0.102} & 0.115 & 0.108 & 0.103 & 0.124 & 0.107 & \textbf{0.102} \\ 
  160 & 0.118 & \textbf{0.105} & \textbf{0.102} & \underline{\textbf{0.113}} & 0.106 & \textbf{0.102} & 0.115 & \textbf{0.105} & \textbf{0.102} & 0.116 & 0.109 & 0.103 & 0.143 & 0.108 & \textbf{0.102} \\ 
  320 & 0.127 & \textbf{0.106} & \textbf{0.102} & \underline{\textbf{0.116}} & \textbf{0.106} & \textbf{0.102} & 0.117 & \textbf{0.106} & \textbf{0.102} & 0.118 & 0.110 & 0.103 & 0.144 & 0.109 & \textbf{0.102} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{RMSE}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{1.507}} & 0.998 & \underline{\textbf{0.665}} & 1.510 & \underline{\textbf{0.950}} & 0.668 & 1.622 & 0.972 & 0.671 & 1.676 & 1.172 & 0.717 & 1.644 & 1.054 & 0.712 \\ 
   40 & \underline{\textbf{2.306}} & \underline{\textbf{1.455}} & \underline{\textbf{0.957}} & 2.486 & 1.466 & 0.963 & 2.513 & 1.458 & 0.967 & 2.585 & 1.794 & 1.064 & 2.548 & 1.643 & 1.020 \\ 
   80 & 3.725 & \underline{\textbf{2.147}} & \underline{\textbf{1.381}} & \underline{\textbf{3.408}} & 2.485 & 1.388 & 3.767 & 2.205 & 1.391 & 3.860 & 2.736 & 1.567 & 5.348 & 2.559 & 1.456 \\ 
  160 & 6.527 & 3.237 & \underline{\textbf{1.989}} & \underline{\textbf{5.212}} & \underline{\textbf{3.147}} & 1.996 & 5.639 & 3.263 & 1.995 & 5.746 & 4.067 & 2.291 & 10.960 & 3.882 & 2.075 \\ 
  320 & 11.706 & 5.126 & 2.870 & \underline{\textbf{7.915}} & \underline{\textbf{4.860}} & 2.879 & 8.357 & 4.999 & \underline{\textbf{2.856}} & 8.468 & 6.141 & 3.342 & 15.421 & 5.972 & 2.953 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Correct sparsity}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   40 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   80 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{True model included}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   40 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   80 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Share of relevant variables}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.096}} & 0.114 & 0.173 & 0.094 & 0.116 & 0.155 & 0.076 & 0.113 & 0.171 & 0.081 & 0.121 & \underline{\textbf{0.196}} & 0.088 & \underline{\textbf{0.123}} & 0.129 \\ 
   40 & \underline{\textbf{0.091}} & 0.110 & 0.162 & 0.069 & 0.108 & 0.141 & 0.059 & 0.105 & 0.158 & 0.061 & 0.109 & \underline{\textbf{0.173}} & 0.065 & \underline{\textbf{0.111}} & 0.120 \\ 
   80 & \underline{\textbf{0.087}} & \underline{\textbf{0.106}} & 0.153 & 0.068 & 0.097 & 0.129 & 0.048 & 0.097 & 0.148 & 0.048 & 0.099 & \underline{\textbf{0.156}} & 0.074 & 0.102 & 0.115 \\ 
  160 & 0.082 & \underline{\textbf{0.104}} & \underline{\textbf{0.145}} & 0.054 & 0.100 & 0.120 & 0.037 & 0.092 & 0.139 & 0.037 & 0.093 & 0.144 & \underline{\textbf{0.096}} & 0.094 & 0.111 \\ 
  320 & \underline{\textbf{0.073}} & \underline{\textbf{0.102}} & \underline{\textbf{0.138}} & 0.041 & 0.095 & 0.113 & 0.027 & 0.085 & 0.131 & 0.027 & 0.085 & 0.134 & 0.068 & 0.087 & 0.109 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Positive Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.012 & 0.007 & 0.003 & 0.013 & 0.007 & 0.002 & \underline{\textbf{0.006}} & \underline{\textbf{0.005}} & 0.002 & 0.008 & 0.007 & 0.005 & 0.013 & 0.009 & \underline{\textbf{0.001}} \\ 
   40 & 0.010 & 0.005 & 0.002 & 0.006 & 0.004 & 0.001 & \underline{\textbf{0.002}} & \underline{\textbf{0.002}} & 0.001 & 0.003 & 0.003 & 0.002 & 0.005 & 0.005 & \underline{\textbf{0.000}} \\ 
   80 & 0.009 & 0.003 & 0.001 & 0.003 & 0.002 & \textbf{0.000} & \textbf{0.001} & \textbf{0.001} & 0.001 & \textbf{0.001} & \textbf{0.001} & 0.001 & 0.024 & 0.002 & \textbf{0.000} \\ 
  160 & 0.009 & 0.003 & 0.001 & 0.001 & 0.001 & \textbf{0.000} & \textbf{0.000} & \underline{\textbf{0.000}} & \textbf{0.000} & \textbf{0.000} & 0.001 & \textbf{0.000} & 0.047 & 0.001 & \textbf{0.000} \\ 
  320 & 0.009 & 0.002 & 0.000 & \textbf{0.000} & \textbf{0.000} & 0.000 & \textbf{0.000} & \textbf{0.000} & 0.000 & \textbf{0.000} & \textbf{0.000} & 0.000 & 0.026 & \textbf{0.000} & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Negative Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.904}} & 0.886 & 0.827 & 0.906 & 0.884 & 0.845 & 0.924 & 0.887 & 0.829 & 0.919 & 0.879 & \underline{\textbf{0.804}} & 0.912 & \underline{\textbf{0.877}} & 0.871 \\ 
   40 & \underline{\textbf{0.909}} & 0.890 & 0.838 & 0.931 & 0.892 & 0.859 & 0.941 & 0.895 & 0.842 & 0.939 & 0.891 & \underline{\textbf{0.827}} & 0.935 & \underline{\textbf{0.889}} & 0.880 \\ 
   80 & \underline{\textbf{0.913}} & \underline{\textbf{0.894}} & 0.847 & 0.932 & 0.903 & 0.871 & 0.952 & 0.903 & 0.852 & 0.952 & 0.901 & \underline{\textbf{0.844}} & 0.926 & 0.898 & 0.885 \\ 
  160 & 0.918 & \underline{\textbf{0.896}} & \underline{\textbf{0.855}} & 0.946 & 0.900 & 0.880 & 0.963 & 0.908 & 0.861 & 0.963 & 0.907 & 0.856 & \underline{\textbf{0.904}} & 0.906 & 0.889 \\ 
  320 & \underline{\textbf{0.927}} & \underline{\textbf{0.898}} & \underline{\textbf{0.862}} & 0.959 & 0.905 & 0.887 & 0.973 & 0.915 & 0.869 & 0.973 & 0.915 & 0.866 & 0.932 & 0.913 & 0.891 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Number of variables}}}\\ 
 \addlinespace[0.5ex]
 20 & 1.088 & 1.207 & 1.758 & 1.076 & 1.224 & 1.569 & 0.821 & 1.174 & 1.733 & 0.893 & 1.288 & 2.011 & 1.005 & 1.320 & 1.303 \\ 
   40 & 1.211 & 1.242 & 1.674 & 0.871 & 1.196 & 1.433 & 0.659 & 1.119 & 1.617 & 0.692 & 1.179 & 1.779 & 0.794 & 1.249 & 1.210 \\ 
   80 & 1.479 & 1.305 & 1.604 & 0.857 & 1.136 & 1.319 & 0.537 & 1.049 & 1.515 & 0.551 & 1.082 & 1.608 & 2.382 & 1.167 & 1.154 \\ 
  160 & 2.169 & 1.420 & 1.558 & 0.709 & 1.124 & 1.229 & 0.411 & 0.990 & 1.428 & 0.419 & 1.007 & 1.482 & 8.063 & 1.083 & 1.120 \\ 
  320 & 3.383 & 1.659 & 1.528 & 0.551 & 1.078 & 1.153 & 0.302 & 0.914 & 1.348 & 0.306 & 0.923 & 1.378 & 8.890 & 1.004 & 1.100 \\ 
   \bottomrule
\end{tabular}
} % end resizebox
\end{table}


==> Tables/tab_MC_BAR_ebic_CMP_rho0_sparsity_r1_eig_0.75_0.25.tex <==
\begin{table}[H]
\centering
\caption{MC simulations: $r$=1, $\rho$=0, EBIC.}
\label{tab:MC_r1_rho0}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc}
  \toprule
 & \multicolumn{3}{c}{\multirow{2}{*}{BAR}}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{\multirow{2}{*}{LASSO}}& \multicolumn{3}{c}{\multirow{2}{*}{SCAD}}\\ 
 & \multicolumn{3}{c}{}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Ridge)}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Lasso)}& \multicolumn{3}{c}{}& \multicolumn{3}{c}{}\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 $T$ & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 \\ 
\midrule 
  \addlinespace
$K$ & \multicolumn{15}{c}{\underline{\textit{RMSFE}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.109}} & \textbf{0.104} & \textbf{0.100} & 0.111 & \textbf{0.104} & \textbf{0.100} & 0.111 & \textbf{0.104} & \textbf{0.100} & 0.111 & 0.106 & \textbf{0.100} & 0.111 & 0.105 & \textbf{0.100} \\ 
   40 & \underline{\textbf{0.112}} & \underline{\textbf{0.103}} & \textbf{0.101} & 0.115 & 0.106 & \textbf{0.101} & 0.113 & 0.104 & \textbf{0.101} & 0.113 & 0.106 & \textbf{0.101} & 0.113 & 0.105 & \textbf{0.101} \\ 
   80 & 0.116 & \underline{\textbf{0.104}} & \textbf{0.100} & \underline{\textbf{0.113}} & 0.112 & \textbf{0.100} & 0.114 & 0.106 & \textbf{0.100} & 0.114 & 0.108 & 0.101 & 0.125 & 0.107 & \textbf{0.100} \\ 
  160 & 0.123 & \textbf{0.106} & \textbf{0.100} & \underline{\textbf{0.114}} & 0.107 & \textbf{0.100} & 0.115 & \textbf{0.106} & \textbf{0.100} & 0.115 & 0.109 & 0.101 & 0.145 & 0.109 & \textbf{0.100} \\ 
  320 & 0.129 & 0.109 & \textbf{0.100} & \textbf{0.116} & 0.110 & 0.101 & \textbf{0.116} & \underline{\textbf{0.108}} & \textbf{0.100} & \textbf{0.116} & 0.110 & 0.101 & 0.143 & 0.110 & \textbf{0.100} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{RMSE}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{1.740}} & 1.006 & 0.223 & 1.900 & 0.993 & 0.221 & 1.824 & \underline{\textbf{0.907}} & 0.214 & 1.857 & 1.234 & 0.468 & 1.847 & 1.091 & \underline{\textbf{0.183}} \\ 
   40 & 2.892 & \underline{\textbf{1.468}} & 0.326 & 3.075 & 1.991 & 0.334 & \underline{\textbf{2.806}} & 1.523 & 0.318 & 2.821 & 1.970 & 0.734 & 2.838 & 1.825 & \underline{\textbf{0.264}} \\ 
   80 & 5.192 & \underline{\textbf{2.289}} & 0.493 & \underline{\textbf{4.122}} & 3.885 & 0.531 & 4.179 & 2.503 & 0.470 & 4.165 & 3.086 & 1.141 & 6.395 & 2.958 & \underline{\textbf{0.398}} \\ 
  160 & 9.414 & \underline{\textbf{3.900}} & 0.744 & 6.203 & 4.163 & 0.952 & 6.125 & 3.928 & 0.684 & \underline{\textbf{6.080}} & 4.682 & 1.745 & 13.573 & 4.581 & \underline{\textbf{0.610}} \\ 
  320 & 15.256 & 7.678 & 1.140 & 9.052 & 7.004 & 2.664 & 8.847 & \underline{\textbf{6.205}} & 0.988 & \underline{\textbf{8.761}} & 7.108 & 2.645 & 18.910 & 7.141 & \underline{\textbf{0.973}} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Correct sparsity}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & \underline{\textbf{0.006}} & 0.410 & 0.000 & 0.000 & 0.582 & 0.000 & 0.002 & 0.434 & 0.000 & 0.000 & 0.116 & 0.000 & 0.000 & \underline{\textbf{0.837}} \\ 
   40 & 0.000 & 0.000 & 0.085 & 0.000 & 0.000 & 0.296 & 0.000 & 0.000 & 0.124 & 0.000 & 0.000 & 0.016 & 0.000 & 0.000 & \underline{\textbf{0.674}} \\ 
   80 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.086 & 0.000 & 0.000 & 0.008 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & \underline{\textbf{0.437}} \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \underline{\textbf{0.123}} \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \underline{\textbf{0.004}} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{True model included}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.117 & 0.991 & 0.000 & \underline{\textbf{0.189}} & \textbf{1.000} & 0.000 & 0.097 & \textbf{1.000} & 0.000 & 0.098 & \textbf{1.000} & 0.000 & 0.118 & \textbf{1.000} \\ 
   40 & 0.000 & \underline{\textbf{0.013}} & 0.989 & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} \\ 
   80 & 0.000 & 0.000 & 0.975 & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} \\ 
  160 & 0.000 & 0.000 & 0.952 & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} \\ 
  320 & 0.000 & 0.000 & 0.894 & 0.000 & 0.000 & 0.016 & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} & 0.000 & 0.000 & \textbf{1.000} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Share of relevant variables}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.575}} & 0.861 & \textbf{1.000} & 0.437 & \underline{\textbf{0.926}} & \textbf{1.000} & 0.425 & 0.894 & \textbf{1.000} & 0.428 & 0.894 & \textbf{1.000} & 0.443 & 0.900 & \textbf{1.000} \\ 
   40 & \underline{\textbf{0.507}} & \underline{\textbf{0.871}} & \textbf{1.000} & 0.175 & 0.753 & \textbf{1.000} & 0.292 & 0.828 & \textbf{1.000} & 0.294 & 0.828 & \textbf{1.000} & 0.305 & 0.835 & \textbf{1.000} \\ 
   80 & \underline{\textbf{0.384}} & \underline{\textbf{0.862}} & \textbf{1.000} & 0.279 & 0.351 & \textbf{1.000} & 0.198 & 0.742 & \textbf{1.000} & 0.199 & 0.742 & \textbf{1.000} & 0.226 & 0.750 & \textbf{1.000} \\ 
  160 & \underline{\textbf{0.210}} & \underline{\textbf{0.826}} & \textbf{1.000} & 0.138 & 0.736 & \textbf{1.000} & 0.118 & 0.662 & \textbf{1.000} & 0.118 & 0.662 & \textbf{1.000} & 0.177 & 0.669 & \textbf{1.000} \\ 
  320 & 0.079 & \underline{\textbf{0.719}} & \textbf{1.000} & 0.047 & 0.541 & 0.988 & 0.066 & 0.560 & \textbf{1.000} & 0.067 & 0.560 & \textbf{1.000} & \underline{\textbf{0.109}} & 0.568 & \textbf{1.000} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Positive Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.016 & \textbf{0.007} & 0.002 & 0.021 & 0.012 & 0.002 & \underline{\textbf{0.007}} & \textbf{0.007} & 0.002 & 0.010 & 0.012 & 0.006 & 0.015 & 0.015 & \underline{\textbf{0.001}} \\ 
   40 & 0.016 & 0.005 & 0.002 & 0.009 & 0.009 & 0.001 & \textbf{0.003} & \underline{\textbf{0.004}} & 0.001 & \textbf{0.003} & 0.005 & 0.003 & 0.006 & 0.007 & \underline{\textbf{0.000}} \\ 
   80 & 0.017 & 0.004 & 0.001 & 0.004 & 0.005 & \textbf{0.000} & \textbf{0.001} & \textbf{0.002} & 0.001 & \textbf{0.001} & \textbf{0.002} & 0.001 & 0.033 & 0.003 & \textbf{0.000} \\ 
  160 & 0.017 & 0.004 & 0.001 & 0.002 & 0.002 & \textbf{0.000} & \textbf{0.000} & \textbf{0.001} & \textbf{0.000} & \textbf{0.000} & \textbf{0.001} & 0.001 & 0.063 & \textbf{0.001} & \textbf{0.000} \\ 
  320 & 0.012 & 0.005 & \textbf{0.000} & 0.001 & 0.001 & 0.001 & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & 0.035 & 0.001 & \textbf{0.000} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Negative Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.425}} & 0.139 & 0.000 & 0.563 & \underline{\textbf{0.074}} & 0.000 & 0.575 & 0.106 & 0.000 & 0.572 & 0.106 & 0.000 & 0.557 & 0.100 & 0.000 \\ 
   40 & \underline{\textbf{0.493}} & \underline{\textbf{0.129}} & 0.000 & 0.825 & 0.247 & 0.000 & 0.708 & 0.172 & 0.000 & 0.706 & 0.172 & 0.000 & 0.695 & 0.165 & 0.000 \\ 
   80 & \underline{\textbf{0.616}} & \underline{\textbf{0.138}} & 0.000 & 0.721 & 0.649 & 0.000 & 0.802 & 0.258 & 0.000 & 0.801 & 0.258 & 0.000 & 0.774 & 0.250 & 0.000 \\ 
  160 & \underline{\textbf{0.790}} & \underline{\textbf{0.174}} & 0.000 & 0.862 & 0.264 & 0.000 & 0.882 & 0.338 & 0.000 & 0.882 & 0.338 & 0.000 & 0.823 & 0.331 & 0.000 \\ 
  320 & 0.921 & \underline{\textbf{0.281}} & \textbf{0.000} & 0.953 & 0.459 & 0.012 & 0.934 & 0.440 & \textbf{0.000} & 0.933 & 0.440 & \textbf{0.000} & \underline{\textbf{0.891}} & 0.432 & \textbf{0.000} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Number of variables}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.881 & 0.992 & 1.046 & 0.834 & 1.159 & 1.029 & 0.566 & 1.027 & 1.044 & 0.617 & 1.120 & 1.117 & 0.725 & 1.181 & 1.010 \\ 
   40 & 1.113 & 1.076 & 1.061 & 0.521 & 1.118 & 1.032 & 0.400 & 0.967 & 1.055 & 0.426 & 1.026 & 1.104 & 0.537 & 1.112 & 1.010 \\ 
   80 & 1.698 & 1.190 & 1.081 & 0.589 & 0.710 & 1.034 & 0.279 & 0.868 & 1.062 & 0.291 & 0.900 & 1.093 & 2.813 & 0.983 & 1.011 \\ 
  160 & 2.844 & 1.425 & 1.107 & 0.407 & 1.022 & 1.048 & 0.172 & 0.769 & 1.066 & 0.176 & 0.786 & 1.082 & 10.224 & 0.848 & 1.013 \\ 
  320 & 3.826 & 2.165 & 1.142 & 0.257 & 0.831 & 1.267 & 0.103 & 0.644 & 1.067 & 0.105 & 0.652 & 1.074 & 11.289 & 0.794 & 1.018 \\ 
   \bottomrule
\end{tabular}
} % end resizebox
\end{table}


==> Tables/tab_MC_BAR_ebic_CMP_rho0_sparsity_r2_eig_0.75_0.25.tex <==
\begin{table}[H]
\centering
\caption{MC simulations: $r$=2, $\rho$=0, EBIC.}
\label{tab:MC_r2_rho0}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc}
  \toprule
 & \multicolumn{3}{c}{\multirow{2}{*}{BAR}}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{\multirow{2}{*}{LASSO}}& \multicolumn{3}{c}{\multirow{2}{*}{SCAD}}\\ 
 & \multicolumn{3}{c}{}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Ridge)}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Lasso)}& \multicolumn{3}{c}{}& \multicolumn{3}{c}{}\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 $T$ & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 \\ 
\midrule 
  \addlinespace
$K$ & \multicolumn{15}{c}{\underline{\textit{RMSFE}}}\\ 
 \addlinespace[0.5ex]
 20 & \textbf{0.112} & 0.106 & \textbf{0.100} & \textbf{0.112} & 0.106 & \textbf{0.100} & 0.114 & \underline{\textbf{0.105}} & \textbf{0.100} & 0.116 & 0.108 & 0.101 & 0.115 & 0.107 & \textbf{0.100} \\ 
   40 & \underline{\textbf{0.114}} & \textbf{0.105} & \textbf{0.101} & 0.117 & 0.107 & \textbf{0.101} & 0.117 & \textbf{0.105} & \textbf{0.101} & 0.119 & 0.109 & 0.102 & 0.118 & 0.108 & \textbf{0.101} \\ 
   80 & 0.117 & \textbf{0.107} & \textbf{0.100} & \underline{\textbf{0.116}} & 0.110 & 0.101 & 0.119 & \textbf{0.107} & \textbf{0.100} & 0.121 & 0.111 & 0.102 & 0.128 & 0.110 & 0.101 \\ 
  160 & 0.123 & \textbf{0.108} & \textbf{0.100} & \underline{\textbf{0.119}} & \textbf{0.108} & 0.101 & 0.122 & \textbf{0.108} & \textbf{0.100} & 0.124 & 0.113 & 0.102 & 0.147 & 0.112 & 0.101 \\ 
  320 & 0.130 & 0.110 & \textbf{0.100} & \underline{\textbf{0.122}} & 0.110 & 0.102 & 0.124 & \underline{\textbf{0.109}} & \textbf{0.100} & 0.126 & 0.115 & 0.102 & 0.148 & 0.114 & 0.101 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{RMSE}}}\\ 
 \addlinespace[0.5ex]
 20 & 1.755 & 1.104 & \underline{\textbf{0.265}} & \underline{\textbf{1.715}} & 1.104 & 0.301 & 1.813 & \underline{\textbf{1.063}} & 0.267 & 1.830 & 1.213 & 0.458 & 1.847 & 1.195 & 0.362 \\ 
   40 & \underline{\textbf{2.761}} & 1.687 & \textbf{0.392} & 2.763 & 1.756 & 0.466 & 2.805 & \underline{\textbf{1.642}} & \textbf{0.392} & 2.817 & 1.912 & 0.718 & 2.843 & 1.862 & 0.614 \\ 
   80 & 4.594 & 2.636 & 0.581 & \underline{\textbf{3.822}} & 2.904 & 0.758 & 4.212 & \underline{\textbf{2.541}} & \underline{\textbf{0.574}} & 4.223 & 2.984 & 1.113 & 5.523 & 2.899 & 1.027 \\ 
  160 & 7.893 & 4.236 & 0.867 & \underline{\textbf{5.814}} & \underline{\textbf{3.710}} & 1.421 & 6.279 & 3.853 & \underline{\textbf{0.838}} & 6.281 & 4.520 & 1.704 & 11.455 & 4.421 & 1.677 \\ 
  320 & 13.137 & 7.099 & 1.303 & \underline{\textbf{8.754}} & \underline{\textbf{5.703}} & 3.339 & 9.244 & 5.916 & \underline{\textbf{1.220}} & 9.220 & 6.855 & 2.586 & 16.419 & 6.772 & 2.661 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Correct sparsity}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & \underline{\textbf{0.414}} & 0.000 & 0.000 & 0.394 & 0.000 & 0.000 & 0.374 & 0.000 & 0.000 & 0.016 & 0.000 & 0.000 & 0.069 \\ 
   40 & 0.000 & 0.000 & 0.100 & 0.000 & 0.000 & \underline{\textbf{0.101}} & 0.000 & 0.000 & 0.080 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.003 \\ 
   80 & 0.000 & 0.000 & \underline{\textbf{0.003}} & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{True model included}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & 0.990 & 0.000 & 0.000 & 0.986 & 0.000 & 0.000 & 0.991 & 0.000 & 0.000 & \underline{\textbf{0.998}} & 0.000 & 0.000 & 0.909 \\ 
   40 & 0.000 & 0.000 & 0.982 & 0.000 & 0.000 & 0.917 & 0.000 & 0.000 & 0.984 & 0.000 & 0.000 & \underline{\textbf{0.996}} & 0.000 & 0.000 & 0.633 \\ 
   80 & 0.000 & 0.000 & 0.938 & 0.000 & 0.000 & 0.555 & 0.000 & 0.000 & 0.948 & 0.000 & 0.000 & \underline{\textbf{0.975}} & 0.000 & 0.000 & 0.186 \\ 
  160 & 0.000 & 0.000 & 0.790 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.833 & 0.000 & 0.000 & \underline{\textbf{0.899}} & 0.000 & 0.000 & 0.002 \\ 
  320 & 0.000 & 0.000 & 0.515 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.568 & 0.000 & 0.000 & \underline{\textbf{0.662}} & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Share of relevant variables}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.477}} & 0.711 & \textbf{1.000} & 0.463 & 0.695 & \textbf{1.000} & 0.420 & 0.730 & \textbf{1.000} & 0.458 & \underline{\textbf{0.798}} & \textbf{1.000} & 0.458 & 0.762 & 0.998 \\ 
   40 & \underline{\textbf{0.447}} & 0.679 & \textbf{1.000} & 0.344 & 0.609 & 0.999 & 0.331 & 0.686 & \textbf{1.000} & 0.354 & \underline{\textbf{0.738}} & \textbf{1.000} & 0.357 & 0.719 & 0.994 \\ 
   80 & \underline{\textbf{0.404}} & 0.645 & \textbf{1.000} & 0.367 & 0.508 & 0.996 & 0.260 & 0.633 & \textbf{1.000} & 0.272 & \underline{\textbf{0.670}} & \textbf{1.000} & 0.296 & 0.663 & 0.990 \\ 
  160 & \underline{\textbf{0.351}} & 0.605 & 0.999 & 0.285 & 0.599 & 0.977 & 0.191 & 0.580 & 0.999 & 0.198 & \underline{\textbf{0.606}} & \underline{\textbf{1.000}} & 0.289 & 0.605 & 0.985 \\ 
  320 & \underline{\textbf{0.293}} & \underline{\textbf{0.563}} & \textbf{0.999} & 0.209 & 0.531 & 0.816 & 0.136 & 0.523 & \textbf{0.999} & 0.139 & 0.540 & \textbf{0.999} & 0.235 & 0.542 & 0.979 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Positive Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.020 & 0.011 & \underline{\textbf{0.002}} & 0.021 & 0.012 & 0.003 & \underline{\textbf{0.010}} & \underline{\textbf{0.009}} & 0.003 & 0.015 & 0.018 & 0.012 & 0.023 & 0.018 & 0.007 \\ 
   40 & 0.016 & 0.008 & \textbf{0.002} & 0.011 & 0.007 & \textbf{0.002} & \underline{\textbf{0.004}} & \underline{\textbf{0.004}} & \textbf{0.002} & 0.006 & 0.008 & 0.005 & 0.010 & 0.009 & 0.004 \\ 
   80 & 0.015 & 0.006 & \textbf{0.001} & 0.005 & 0.005 & \textbf{0.001} & \textbf{0.002} & \underline{\textbf{0.002}} & \textbf{0.001} & \textbf{0.002} & 0.003 & 0.002 & 0.023 & 0.004 & 0.002 \\ 
  160 & 0.013 & 0.005 & \textbf{0.001} & 0.002 & 0.002 & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & \textbf{0.001} & 0.047 & 0.002 & \textbf{0.001} \\ 
  320 & 0.010 & 0.005 & \textbf{0.000} & 0.001 & 0.001 & 0.001 & \textbf{0.000} & \underline{\textbf{0.000}} & \textbf{0.000} & \textbf{0.000} & 0.001 & \textbf{0.000} & 0.028 & 0.001 & \textbf{0.000} \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Negative Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.523}} & 0.289 & \textbf{0.000} & 0.537 & 0.305 & \textbf{0.000} & 0.580 & 0.270 & \textbf{0.000} & 0.542 & \underline{\textbf{0.202}} & \textbf{0.000} & 0.542 & 0.238 & 0.002 \\ 
   40 & \underline{\textbf{0.553}} & 0.321 & \textbf{0.000} & 0.656 & 0.391 & 0.001 & 0.669 & 0.314 & \textbf{0.000} & 0.646 & \underline{\textbf{0.262}} & \textbf{0.000} & 0.643 & 0.281 & 0.006 \\ 
   80 & \underline{\textbf{0.596}} & 0.355 & \textbf{0.000} & 0.633 & 0.492 & 0.004 & 0.740 & 0.367 & \textbf{0.000} & 0.728 & \underline{\textbf{0.330}} & \textbf{0.000} & 0.704 & 0.337 & 0.010 \\ 
  160 & \underline{\textbf{0.649}} & 0.395 & 0.001 & 0.715 & 0.401 & 0.023 & 0.809 & 0.420 & 0.001 & 0.802 & \underline{\textbf{0.394}} & \underline{\textbf{0.000}} & 0.711 & 0.395 & 0.015 \\ 
  320 & \underline{\textbf{0.707}} & \underline{\textbf{0.437}} & \textbf{0.001} & 0.791 & 0.469 & 0.184 & 0.864 & 0.477 & \textbf{0.001} & 0.861 & 0.460 & \textbf{0.001} & 0.765 & 0.458 & 0.021 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Number of variables}}}\\ 
 \addlinespace[0.5ex]
 20 & 1.307 & 1.620 & 2.043 & 1.309 & 1.599 & 2.046 & 1.014 & 1.614 & 2.049 & 1.194 & 1.914 & 2.209 & 1.333 & 1.848 & 2.129 \\ 
   40 & 1.517 & 1.667 & 2.062 & 1.122 & 1.493 & 2.056 & 0.817 & 1.542 & 2.066 & 0.926 & 1.766 & 2.195 & 1.101 & 1.779 & 2.148 \\ 
   80 & 1.951 & 1.787 & 2.084 & 1.096 & 1.378 & 2.071 & 0.647 & 1.433 & 2.080 & 0.708 & 1.589 & 2.180 & 2.424 & 1.664 & 2.153 \\ 
  160 & 2.772 & 2.030 & 2.112 & 0.903 & 1.454 & 2.089 & 0.474 & 1.311 & 2.091 & 0.506 & 1.418 & 2.169 & 8.078 & 1.517 & 2.137 \\ 
  320 & 3.751 & 2.570 & 2.149 & 0.699 & 1.333 & 1.867 & 0.336 & 1.181 & 2.098 & 0.353 & 1.251 & 2.155 & 9.226 & 1.376 & 2.101 \\ 
   \bottomrule
\end{tabular}
} % end resizebox
\end{table}


==> Tables/tab_MC_BAR_ebic_CMP_rho0_sparsity_r5_eig_0.75_0.25.tex <==
\begin{table}[H]
\centering
\caption{MC simulations: $r$=5, $\rho$=0, EBIC.}
\label{tab:MC_r5_rho0}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc}
  \toprule
 & \multicolumn{3}{c}{\multirow{2}{*}{BAR}}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{Adaptive LASSO}& \multicolumn{3}{c}{\multirow{2}{*}{LASSO}}& \multicolumn{3}{c}{\multirow{2}{*}{SCAD}}\\ 
 & \multicolumn{3}{c}{}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Ridge)}& \multicolumn{3}{c}{(1\textsuperscript{st} step: Lasso)}& \multicolumn{3}{c}{}& \multicolumn{3}{c}{}\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
 $T$ & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 & 50 & 100 & 500 \\ 
\midrule 
  \addlinespace
$K$ & \multicolumn{15}{c}{\underline{\textit{RMSFE}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.114}} & \textbf{0.108} & \textbf{0.101} & 0.115 & \textbf{0.108} & \textbf{0.101} & 0.117 & 0.109 & \textbf{0.101} & 0.117 & 0.111 & 0.102 & 0.117 & 0.110 & \textbf{0.101} \\ 
   40 & \underline{\textbf{0.116}} & \underline{\textbf{0.108}} & \textbf{0.101} & 0.118 & 0.109 & 0.102 & 0.119 & 0.110 & \textbf{0.101} & 0.119 & 0.112 & 0.103 & 0.119 & 0.111 & 0.102 \\ 
   80 & 0.119 & \underline{\textbf{0.109}} & \textbf{0.101} & \underline{\textbf{0.118}} & 0.113 & 0.102 & 0.120 & 0.112 & \textbf{0.101} & 0.120 & 0.114 & 0.103 & 0.133 & 0.114 & 0.102 \\ 
  160 & 0.125 & \underline{\textbf{0.110}} & \textbf{0.101} & \underline{\textbf{0.119}} & 0.111 & 0.102 & 0.121 & 0.113 & \textbf{0.101} & 0.121 & 0.115 & 0.103 & 0.154 & 0.115 & 0.102 \\ 
  320 & 0.134 & \underline{\textbf{0.112}} & \textbf{0.101} & \underline{\textbf{0.121}} & 0.113 & 0.102 & 0.122 & 0.114 & \textbf{0.101} & 0.122 & 0.117 & 0.104 & 0.152 & 0.116 & 0.103 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{RMSE}}}\\ 
 \addlinespace[0.5ex]
 20 & 1.956 & \underline{\textbf{1.357}} & 0.533 & \underline{\textbf{1.953}} & 1.376 & 0.555 & 2.079 & 1.480 & \underline{\textbf{0.524}} & 2.044 & 1.578 & 0.691 & 2.046 & 1.525 & 0.598 \\ 
   40 & \underline{\textbf{2.977}} & \underline{\textbf{2.020}} & 0.779 & 2.999 & 2.172 & 0.838 & 3.088 & 2.286 & \underline{\textbf{0.769}} & 3.044 & 2.442 & 1.094 & 3.047 & 2.377 & 0.939 \\ 
   80 & 4.762 & \underline{\textbf{3.041}} & 1.136 & \underline{\textbf{4.255}} & 3.552 & 1.275 & 4.504 & 3.492 & \underline{\textbf{1.128}} & 4.447 & 3.705 & 1.695 & 6.346 & 3.638 & 1.469 \\ 
  160 & 8.066 & \underline{\textbf{4.652}} & 1.661 & \underline{\textbf{6.268}} & 4.827 & 1.975 & 6.513 & 5.195 & \underline{\textbf{1.654}} & 6.441 & 5.479 & 2.581 & 12.516 & 5.420 & 2.272 \\ 
  320 & 13.618 & 7.414 & \underline{\textbf{2.437}} & \underline{\textbf{9.131}} & \underline{\textbf{7.294}} & 3.232 & 9.340 & 7.758 & 2.441 & 9.249 & 8.101 & 3.906 & 17.162 & 8.121 & 3.491 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Correct sparsity}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   40 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   80 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{True model included}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   40 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   80 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  320 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Share of relevant variables}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.208}} & 0.347 & 0.590 & 0.182 & \underline{\textbf{0.349}} & 0.606 & 0.129 & 0.304 & 0.606 & 0.137 & 0.326 & \underline{\textbf{0.666}} & 0.155 & 0.343 & 0.625 \\ 
   40 & \underline{\textbf{0.192}} & \underline{\textbf{0.328}} & 0.579 & 0.114 & 0.294 & 0.585 & 0.086 & 0.252 & 0.592 & 0.089 & 0.263 & \underline{\textbf{0.638}} & 0.099 & 0.279 & 0.604 \\ 
   80 & \underline{\textbf{0.172}} & \underline{\textbf{0.310}} & 0.569 & 0.103 & 0.216 & 0.565 & 0.057 & 0.205 & 0.580 & 0.059 & 0.210 & \underline{\textbf{0.615}} & 0.103 & 0.222 & 0.584 \\ 
  160 & \underline{\textbf{0.150}} & \underline{\textbf{0.291}} & 0.559 & 0.068 & 0.228 & 0.541 & 0.036 & 0.170 & 0.567 & 0.037 & 0.173 & \underline{\textbf{0.594}} & 0.139 & 0.180 & 0.566 \\ 
  320 & \underline{\textbf{0.122}} & \underline{\textbf{0.271}} & 0.550 & 0.042 & 0.189 & 0.505 & 0.023 & 0.136 & 0.555 & 0.023 & 0.137 & \underline{\textbf{0.575}} & 0.095 & 0.143 & 0.549 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Positive Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & 0.016 & 0.009 & \underline{\textbf{0.003}} & 0.015 & 0.013 & 0.006 & \underline{\textbf{0.005}} & \underline{\textbf{0.007}} & 0.005 & 0.008 & 0.013 & 0.021 & 0.014 & 0.018 & 0.012 \\ 
   40 & 0.013 & 0.006 & \underline{\textbf{0.002}} & 0.006 & 0.007 & 0.003 & \textbf{0.002} & \underline{\textbf{0.003}} & 0.003 & \textbf{0.002} & 0.005 & 0.009 & 0.005 & 0.007 & 0.006 \\ 
   80 & 0.011 & 0.005 & \underline{\textbf{0.001}} & 0.002 & 0.003 & 0.002 & \textbf{0.001} & \underline{\textbf{0.001}} & 0.002 & \textbf{0.001} & 0.002 & 0.004 & 0.034 & 0.003 & 0.003 \\ 
  160 & 0.012 & 0.004 & \textbf{0.001} & 0.001 & 0.001 & \textbf{0.001} & \textbf{0.000} & \underline{\textbf{0.000}} & \textbf{0.001} & \textbf{0.000} & 0.001 & 0.002 & 0.061 & 0.001 & \textbf{0.001} \\ 
  320 & 0.010 & 0.003 & 0.001 & \textbf{0.000} & 0.001 & 0.001 & \textbf{0.000} & \textbf{0.000} & \underline{\textbf{0.000}} & \textbf{0.000} & \textbf{0.000} & 0.001 & 0.032 & 0.001 & 0.001 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{False Negative Rate}}}\\ 
 \addlinespace[0.5ex]
 20 & \underline{\textbf{0.792}} & 0.653 & 0.410 & 0.818 & \underline{\textbf{0.651}} & 0.394 & 0.871 & 0.696 & 0.394 & 0.863 & 0.674 & \underline{\textbf{0.334}} & 0.845 & 0.657 & 0.375 \\ 
   40 & \underline{\textbf{0.808}} & \underline{\textbf{0.672}} & 0.421 & 0.886 & 0.706 & 0.415 & 0.914 & 0.748 & 0.408 & 0.911 & 0.737 & \underline{\textbf{0.362}} & 0.901 & 0.721 & 0.396 \\ 
   80 & \underline{\textbf{0.828}} & \underline{\textbf{0.690}} & 0.431 & 0.897 & 0.784 & 0.435 & 0.943 & 0.795 & 0.420 & 0.941 & 0.790 & \underline{\textbf{0.385}} & 0.897 & 0.778 & 0.416 \\ 
  160 & \underline{\textbf{0.850}} & \underline{\textbf{0.709}} & 0.441 & 0.932 & 0.772 & 0.459 & 0.964 & 0.830 & 0.433 & 0.963 & 0.827 & \underline{\textbf{0.406}} & 0.861 & 0.820 & 0.434 \\ 
  320 & \underline{\textbf{0.878}} & \underline{\textbf{0.729}} & 0.450 & 0.958 & 0.811 & 0.495 & 0.977 & 0.864 & 0.445 & 0.977 & 0.863 & \underline{\textbf{0.425}} & 0.905 & 0.857 & 0.451 \\ 
   \addlinespace
{} & \multicolumn{15}{c}{\underline{\textit{Number of variables}}}\\ 
 \addlinespace[0.5ex]
 20 & 1.277 & 1.868 & 2.993 & 1.141 & 1.938 & 3.114 & 0.729 & 1.629 & 3.100 & 0.802 & 1.831 & 3.648 & 0.982 & 1.982 & 3.305 \\ 
   40 & 1.397 & 1.866 & 2.958 & 0.790 & 1.703 & 3.023 & 0.495 & 1.363 & 3.051 & 0.528 & 1.475 & 3.492 & 0.657 & 1.632 & 3.216 \\ 
   80 & 1.716 & 1.901 & 2.939 & 0.700 & 1.326 & 2.940 & 0.334 & 1.117 & 3.012 & 0.348 & 1.177 & 3.354 & 3.030 & 1.300 & 3.131 \\ 
  160 & 2.544 & 2.010 & 2.922 & 0.496 & 1.336 & 2.840 & 0.212 & 0.925 & 2.965 & 0.218 & 0.958 & 3.234 & 10.098 & 1.042 & 3.044 \\ 
  320 & 3.780 & 2.342 & 2.924 & 0.333 & 1.128 & 2.707 & 0.135 & 0.738 & 2.911 & 0.138 & 0.756 & 3.118 & 10.441 & 0.905 & 2.956 \\ 
   \bottomrule
\end{tabular}
} % end resizebox
\end{table}

